AnyMorph: Learning Transferable Polices By Inferring Agent Morphology

The prototypical approach to reinforcement learning involves training policies tailored to a particular agent from scratch for every new morphology. Recent work aims to eliminate the re-training of policies by investigating whether a morphology-agnostic policy, trained on a diverse set of agents with similar task objectives, can be transferred to new agents with unseen morphologies without re-training. This is a challenging problem that required previous approaches to use hand-designed descriptions of the new agent's morphology. Instead of hand-designing this description, we propose a data-driven method that learns a representation of morphology directly from the reinforcement learning objective. Ours is the first reinforcement learning algorithm that can train a policy to generalize to new agent morphologies without requiring a description of the agent's morphology in advance. We evaluate our approach on the standard benchmark for agent-agnostic control, and improve over the current state of the art in zero-shot generalization to new agents. Importantly, our method attains good performance without an explicit description of morphology.

==> sections/experiments_five.tex <==

outline:

- introduce the goal of this section with a question: "how well does our model perform given only image observations"

- defining the problem statement (given a fixed image-encoder, training a policy agnostic to morphology? Could we also define a problem of generalizing to different image-encoders with different latent spaces? the latter may be harder)

- summarize the results

%\begin{figure*}[htbp]
%    \centering
%    \includegraphics[width=\linewidth]{assets/section_three.pdf}
%    \caption{TODO, replace this with one that contains the complete runs of all baselines.}
%    \label{fig:my_label}
%\end{figure*}

==> sections/experiments_four.tex <==

outline:

- introduce the goal of this section with a question: "how well does our model perform when nothing about morphology is known in advance?"

- description of the how the algorithm is applied in this setting (elaborate on a morphology encoder)

- summarize the results


==> sections/intro.tex <==


% What is the problem?
% People are very skilled at adjusting to changed in dynamics. Often these changes come in the form of changing our morphology, putting on skates, skis, 
% Generalization in RL is very limited. 
Reinforcement learning policies are often trained to perform well on a single task and perform poorly when transferred to a new tasks. Having to learn a new policy for every combination of agent morphology, reward function and dynamics model is expensive. A method that could not only train a single policy across a collection of agent but that could also improve sample efficiency by sharing experience across policies will provide important advancements in terms of policy generalization and as a consequence, training efficiency.

Generalizing to various types of morphology poses unique challenges for policy training. In this instance the algorithm needs to not only be robust to changes in the size of the state and action space, but also the ordering of the items in the state feature vectors. This quickly becomes a combinatorial routing problem~\citep{rosenbaum2018routing}. If we can instead learn a model that can understand this routing given limited information 
%%GB.1.24.22: We should provide a little more information on this type of information.
we can train this richer class of policies that can solve tasks for novel agent morphologies that we are yet to create.

% We need a way to infer the morphology from interaction. This will be the most general method that can also be used outside of simulation.

% edit this, it is just the abstract right now
\begin{figure}
    \centering
    \includegraphics[trim={0.0cm 0.0cm 0.0cm 35.0cm},clip,width=\linewidth]{assets/morphologies}
    \includegraphics[width=\linewidth]{assets/policy_architecture.pdf}
    \caption{Visualization of the architecture of the policy for an example reinforcement learning agent with a seven-dimensional (7d) observation space and a five-dimensional (5d) action space. The policy is invariant to the dimensionality of both the action space and observation space of the task, without making structural assumptions about how sensors and actuators are connected.}
    \label{fig:policy_architecture}
\end{figure}

% Why is it hard?
% This type of generalization requires that network models learning modules that are not only independent of morphology but also of task
% There are many different types of morphology's with slightly different dynamics.
% It is well understood how the dynamics of a robot work if expressed in ridged body physics.
% However, we don't often have information needed to fill in all the blanks for the ridged body system or any general system.
% Inferring this system is hard for ... reason

% How could we make a more general solution to this?
%%GB.1.24.22: This needs a fair bit of work. But the methods section needs to be written before we can describe the important parts of the method here.
To make progress on learning more generalizable policies we need a way to infer the morphology of the agent from only interaction in the environment. This requires 
(1) A way to enable easier learning of the tokenization using an encoder...
%%GB.1.27.22: Need some details on how the matrix learning you are doing works and is a good idea.
the \todo{How does the tokenization and learning the matricies work?}
(2) A model that can process variable length state input and process this state input in such a way to enable adaptability to variable morphology descriptions. In this work we invoke the success of recent Transformer-based methods to translate the routing problem into one of sentence translation. The policy architecture is shown in~\autoref{fig:policy_architecture}, where an example of the transformer architecture processing a 7d observation is shown.

%% Describe how our proposed method is a very good example of the doing the more general solution
%% Brandon will know this better


Using our combination of inferring the state tokenization and using transformers for translating the morphology, we are able to show significant performance gains in data efficiency and policy generalization. 
In particular we achieve larger gains over prior methods as the number of agent morphologies used to train the transformer-based policy are increased. This progress is achieved while requiring less information about the agents morphology compared to prior methods.
% Our method can also train over new types of dynamics that are not restricted to the ridged body paradigm \todo{image-based inputs}.



